Command R7B Arabic: A Small, Enterprise Focused, Multilingual, and Culturally Aware Arabic LLM

Building high-quality large language models (LLMs) for enterprise Arabic applications remains challenging due to the limited availability of digitized Arabic data. In this work, we present a data synthesis and refinement strategy to help address this problem, namely, by leveraging synthetic data generation and human-in-the-loop annotation to expand our Arabic training corpus. We further present our iterative post training recipe that is essential to achieving state-of-the-art performance in aligning the model with human preferences, a critical aspect to enterprise use cases. The culmination of this effort is the release of a small, 7B, open-weight model that outperforms similarly sized peers in head-to-head comparisons and on Arabic-focused benchmarks covering cultural knowledge, instruction following, RAG, and contextual faithfulness.

==> tables/evals_selected.tex <==
\begin{table}
  \centering
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{lccc}
      \toprule
      \textbf{Benchmark} & \textbf{R7B Arabic} & \textbf{R7B} & \textbf{Gemma 9B} \\
      \midrule
      AlGhafa-Native & \textbf{82.2} & 81.5 & 81.3 \\
      Arabic MMLU & 60.9 & 59.7 & \textbf{62.4} \\
      IFEval AR & \textbf{69.0} & 57.8 & 67.8 \\
      TyDI QA Arabic & \textbf{83.0} & 79.9 & 76.4 \\
      FaithEval Arabic* & \textbf{51.6} & 49.9 & 47.0 \\
      \midrule
      \textbf{Average} & \textbf{69.3} & 65.8 & 67.0 \\
      \bottomrule
      \multicolumn{4}{l}{\small *???} \\
    \end{tabular}
  }
  \caption{Performance comparison of selected models on Arabic-specific benchmarks. The highest score in each row is in \textbf{bold}.}
  \label{tab:arabic_models_selected}
\end{table}
